Investigating the effect of electronic correlation on transport properties and phononic states of Vanadium

In the present work, we have tried to investigate the importance of electronic correlation on transport properties and phononic states of Vanadium (V). The temperature-dependent electrical resistivity ($\rho$) and electronic part of thermal conductivity ($\kappa_e$) due to electron-electron interactions (EEIs) and electron-phonon interactions (EPIs) are computed. The values of $\rho$ due to EEIs are found to be extremely small in comparison to $\rho$ due to EPIs. For instance, at 300 K, the calculated value of $\rho$ due to EEIs (EPIs) is $\sim$ 0.859$\times10^{-3}$ ($\sim$ 0.20) $\mu\Omega$m. The magnitudes of $\kappa_e$ due to EPIs are found to be in good agreement with the experimental results. These observations indicate the negligible importance of EEIs to these quantities for V. However, at 300 K, the value of Seebeck coefficient ($S$) at DFT+DMFT level ($\sim$ -0.547 $\mu$VK$^{-1}$) is found to be entirely different than at DFT level ($\sim 7.401$ $\mu$VK$^{-1}$). Also, the DFT+DMFT value of $S$ at 300 K is in good match with the available experimental data (-1.06 $\mu$VK$^{-1}$, 1.0 $\mu$VK$^{-1}$). Apart from this, the study of phononic states at DFT and DFT+DMFT level is performed. The obtained phononic band structure and phonon DOS at DFT+DMFT differ to a good extent from that at DFT. The maximum energy of phononic state obtained at DFT (DFT+DMFT) is $\sim$ 33.83 ($\sim$ 35.15) meV, where the result of DFT+DMFT is obtained more closer to the experimental data (35.15, 36.98 & 41.77 meV). These results highlight the importance of electronic correlation on $S$ & phononic states of simple correlated V metal.

==> Figure_eps/Resistivity_300K_new <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Fri Apr 21 18:51:50 2023"
@with string
@    string on
@    string loctype view
@    string 0.871323529412, 0.939950980392
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.000000
@    string def "(a)"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world -1, -0.0005, 301, 0.301
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.334559, 0.959559, 0.974265
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "\f{Times-Italic}T\f{} (K)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.250000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 20
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 0.700000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.350000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\f{Symbol}r\f{} (\xm W\f{Times-Roman} m)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.250000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.05
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 0.700000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.350000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.200000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.172303922, 0.959313725
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden true
@    s0 type xy
@    s0 symbol 1
@    s0 symbol size 0.750000
@    s0 symbol color 4
@    s0 symbol pattern 1
@    s0 symbol fill color 4
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 4
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 4
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 4
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "Cols 1:3"
@    s0 legend  "Our Work"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 1
@    s1 symbol size 0.750000
@    s1 symbol color 4
@    s1 symbol pattern 1
@    s1 symbol fill color 4
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 4
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 4
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "Cols 1:2"
@    s1 legend  "\x\r\s\f{Times-Roman}eph\N"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 10
@    s2 symbol size 0.750000
@    s2 symbol color 1
@    s2 symbol pattern 1
@    s2 symbol fill color 1
@    s2 symbol fill pattern 0
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 0
@    s2 line linewidth 1.0
@    s2 line color 1
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 1
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "Cols 1:2"
@    s2 legend  "Exp. 1 [26]"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 7
@    s3 symbol size 0.750000
@    s3 symbol color 8
@    s3 symbol pattern 1
@    s3 symbol fill color 8
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 0
@    s3 line linewidth 1.0
@    s3 line color 8
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 8
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "copy of set G0.S5"
@    s3 legend  "Exp. 2 [27]"
@    s4 hidden false
@    s4 type xy
@    s4 symbol 2
@    s4 symbol size 0.750000
@    s4 symbol color 15
@    s4 symbol pattern 1
@    s4 symbol fill color 15
@    s4 symbol fill pattern 1
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 0
@    s4 line linewidth 1.0
@    s4 line color 15
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 15
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "Cols 1:2"
@    s4 legend  "Exp. 3 [28]"
@    s5 hidden false
@    s5 type xy
@    s5 symbol 4
@    s5 symbol size 0.750000
@    s5 symbol color 2
@    s5 symbol pattern 1
@    s5 symbol fill color 2
@    s5 symbol fill pattern 1
@    s5 symbol linewidth 1.0
@    s5 symbol linestyle 1
@    s5 symbol char 65
@    s5 symbol char font 0
@    s5 symbol skip 0
@    s5 line type 1
@    s5 line linestyle 0
@    s5 line linewidth 1.0
@    s5 line color 2
@    s5 line pattern 1
@    s5 baseline type 0
@    s5 baseline off
@    s5 dropline off
@    s5 fill type 0
@    s5 fill rule 0
@    s5 fill color 1
@    s5 fill pattern 1
@    s5 avalue off
@    s5 avalue type 2
@    s5 avalue char size 1.000000
@    s5 avalue font 0
@    s5 avalue color 1
@    s5 avalue rot 0
@    s5 avalue format general
@    s5 avalue prec 3
@    s5 avalue prepend ""
@    s5 avalue append ""
@    s5 avalue offset 0.000000 , 0.000000
@    s5 errorbar on
@    s5 errorbar place both
@    s5 errorbar color 2
@    s5 errorbar pattern 1
@    s5 errorbar size 1.000000
@    s5 errorbar linewidth 1.0
@    s5 errorbar linestyle 1
@    s5 errorbar riser linewidth 1.0
@    s5 errorbar riser linestyle 1
@    s5 errorbar riser clip off
@    s5 errorbar riser clip length 0.100000
@    s5 comment "copy of set G0.S6"
@    s5 legend  "Exp. 4 [29]"
@target G0.S0
@type xy
2 6.5387548e-07
20 0.00070140216
40 0.0043500765
60 0.013419188
80 0.026613234
100 0.041610955
120 0.057137024
140 0.072670845
160 0.088033348
180 0.10318132
200 0.11812157
220 0.13287693
240 0.1474731
260 0.16193401
280 0.1762804
300 0.19052974
&
@target G0.S1
@type xy
2 8.1577725e-08
20 0.00042030777
40 0.0043079041
60 0.015029891
80 0.029838643
100 0.046028399
120 0.062443109
140 0.078696957
160 0.094693093
180 0.11043264
200 0.1259456
220 0.14126675
240 0.15642795
260 0.17145618
280 0.18637359
300 0.2011982
&
@target G0.S2
@type xy
5.2 0.0092
65 0.0244
129 0.0847
229 0.1714
&
@target G0.S3
@type xy
5 0.0082
20 0.0082
40 0.013
60 0.021
80 0.034
121 0.074
161 0.112
201 0.145
241 0.178
280 0.209
300 0.225
&
@target G0.S4
@type xy
25.1 0.0069
38.9 0.0104
57.1 0.0198
82.2 0.0418
100.4 0.0615
120.8 0.0858
139 0.107
161.8 0.134
182.2 0.159
200.4 0.177
220.9 0.197
243.7 0.212
259.6 0.234
282.4 0.258
300 0.2769
&
@target G0.S5
@type xy
1 0.0001
20 0.000391
40 0.00304
60 0.01114
80 0.02413
100 0.0401
150 0.0822
200 0.1243
250 0.1637
273 0.1814
293 0.1968
300 0.2021
&


==> Figure_eps/Rho_ep_ee_edit <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Fri Apr 21 18:50:53 2023"
@with string
@    string on
@    string loctype world
@    string g0
@    string 919.658622909, 0.755217391481
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.000000
@    string def "(b)"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 300, 0.2, 1000, 0.8
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.371324, 0.982843, 0.963235
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "\f{Times-Italic}T\f{} (K)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.250000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 100
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 0.700000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.350000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.200000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\f{Symbol}r\f{} (\xm W\f{Times-Roman} m)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.250000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.1
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 0.700000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.350000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.200000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype world
@    legend 315, 0.79
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 1
@    s0 symbol size 0.750000
@    s0 symbol color 4
@    s0 symbol pattern 1
@    s0 symbol fill color 4
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 4
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 4
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "Cols 1:3"
@    s0 legend  "\x\r\s\f{Times-Roman}eph\N"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 10
@    s1 symbol size 0.900000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 0
@    s1 line linewidth 1.0
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "/home/prakash/Desktop/Resistivity/300-1000K/A. Chemoplekov, G. Kh. Panova"
@    s1 legend  "Exp. 1 [26]"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 0.900000
@    s2 symbol color 6
@    s2 symbol pattern 1
@    s2 symbol fill color 6
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 0
@    s2 line linewidth 1.0
@    s2 line color 6
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 6
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "/home/prakash/Desktop/Resistivity/300-1000K/Bass.dat"
@    s2 legend  "Exp. 2 [25]"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 4
@    s3 symbol size 0.900000
@    s3 symbol color 2
@    s3 symbol pattern 1
@    s3 symbol fill color 2
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 0
@    s3 line linewidth 1.0
@    s3 line color 2
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 2
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "/home/prakash/Desktop/Resistivity/300-1000K/desai"
@    s3 legend  "Exp. 3 [29]"
@    s4 hidden true
@    s4 type xy
@    s4 symbol 1
@    s4 symbol size 0.500000
@    s4 symbol color 4
@    s4 symbol pattern 1
@    s4 symbol fill color 4
@    s4 symbol fill pattern 1
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 1
@    s4 line linewidth 1.0
@    s4 line color 4
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 4
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "Cols 1:3"
@    s4 legend  "Our Work"
@    s5 hidden true
@    s5 type xy
@    s5 symbol 1
@    s5 symbol size 0.500000
@    s5 symbol color 4
@    s5 symbol pattern 1
@    s5 symbol fill color 4
@    s5 symbol fill pattern 2
@    s5 symbol linewidth 1.0
@    s5 symbol linestyle 1
@    s5 symbol char 65
@    s5 symbol char font 0
@    s5 symbol skip 0
@    s5 line type 1
@    s5 line linestyle 1
@    s5 line linewidth 1.0
@    s5 line color 4
@    s5 line pattern 1
@    s5 baseline type 0
@    s5 baseline off
@    s5 dropline off
@    s5 fill type 0
@    s5 fill rule 0
@    s5 fill color 1
@    s5 fill pattern 1
@    s5 avalue off
@    s5 avalue type 2
@    s5 avalue char size 1.000000
@    s5 avalue font 0
@    s5 avalue color 1
@    s5 avalue rot 0
@    s5 avalue format general
@    s5 avalue prec 3
@    s5 avalue prepend ""
@    s5 avalue append ""
@    s5 avalue offset 0.000000 , 0.000000
@    s5 errorbar on
@    s5 errorbar place both
@    s5 errorbar color 4
@    s5 errorbar pattern 1
@    s5 errorbar size 1.000000
@    s5 errorbar linewidth 1.0
@    s5 errorbar linestyle 1
@    s5 errorbar riser linewidth 1.0
@    s5 errorbar riser linestyle 1
@    s5 errorbar riser clip off
@    s5 errorbar riser clip length 0.100000
@    s5 comment "Cols 1:2"
@    s5 legend  "Our Work (\x r\s\f{Times-Roman}eph\N)"
@    s6 hidden true
@    s6 type xy
@    s6 symbol 1
@    s6 symbol size 0.900000
@    s6 symbol color 4
@    s6 symbol pattern 1
@    s6 symbol fill color 4
@    s6 symbol fill pattern 1
@    s6 symbol linewidth 1.0
@    s6 symbol linestyle 1
@    s6 symbol char 65
@    s6 symbol char font 0
@    s6 symbol skip 0
@    s6 line type 1
@    s6 line linestyle 1
@    s6 line linewidth 1.0
@    s6 line color 4
@    s6 line pattern 1
@    s6 baseline type 0
@    s6 baseline off
@    s6 dropline off
@    s6 fill type 0
@    s6 fill rule 0
@    s6 fill color 1
@    s6 fill pattern 1
@    s6 avalue off
@    s6 avalue type 2
@    s6 avalue char size 1.000000
@    s6 avalue font 0
@    s6 avalue color 1
@    s6 avalue rot 0
@    s6 avalue format general
@    s6 avalue prec 3
@    s6 avalue prepend ""
@    s6 avalue append ""
@    s6 avalue offset 0.000000 , 0.000000
@    s6 errorbar on
@    s6 errorbar place both
@    s6 errorbar color 4
@    s6 errorbar pattern 1
@    s6 errorbar size 1.000000
@    s6 errorbar linewidth 1.0
@    s6 errorbar linestyle 1
@    s6 errorbar riser linewidth 1.0
@    s6 errorbar riser linestyle 1
@    s6 errorbar riser clip off
@    s6 errorbar riser clip length 0.100000
@    s6 comment "Cols 1:4"
@    s6 legend  "Our Work (\x r\s\f{Times-Roman}ee\N+ \x\r\s\f{Times-Roman}eph\N)"
@target G0.S0
@type xy
300 0.2011982
320 0.21594463
340 0.23062474
360 0.24524824
380 0.25982311
400 0.27435594
420 0.28885221
440 0.30331652
460 0.31775274
480 0.33216415
500 0.34655357
520 0.36092337
540 0.37527564
560 0.38961217
580 0.40393451
600 0.41824403
620 0.43254192
640 0.44682923
660 0.46110689
680 0.47537572
700 0.48963647
720 0.50388979
740 0.51813625
760 0.5323764
780 0.54661071
800 0.56083959
820 0.57506345
840 0.58928263
860 0.60349746
880 0.61770822
900 0.63191519
920 0.6461186
940 0.66031867
960 0.67451563
980 0.68870964
1000 0.70290089
&
@target G0.S1
@type xy
337 0.254
409 0.3
530 0.39
659 0.469
789 0.545
875 0.605
975 0.654
&
@target G0.S2
@type xy
309.6 0.2229
333.6 0.2409
349.6 0.2532
373 0.27
573 0.402
773 0.521
973 0.628
&
@target G0.S3
@type xy
300 0.2021
350 0.242
400 0.28
500 0.349
600 0.412
700 0.474
800 0.534
900 0.591
1000 0.646
&
@target G0.S4
@type xy
300 0.19052974
320 0.20469655
340 0.21879285
360 0.2328286
380 0.24681206
400 0.26075015
420 0.27464865
440 0.28851243
460 0.30234562
480 0.31615175
500 0.32993382
520 0.34369442
540 0.35743579
560 0.37115987
580 0.38486835
600 0.39856272
620 0.41224428
640 0.42591417
660 0.43957342
680 0.45322292
700 0.46686349
720 0.48049584
740 0.49412062
760 0.5077384
780 0.52134972
800 0.53495504
820 0.54855478
840 0.56214934
860 0.57573908
880 0.5893243
900 0.60290531
920 0.61648238
940 0.63005575
960 0.64362565
980 0.65719229
1000 0.67075586
&
@target G0.S5
@type xy
300 0.2011982
400 0.27435594
500 0.34655357
600 0.41824403
700 0.48963647
800 0.56083959
900 0.63191519
1000 0.70290089
&
@target G0.S6
@type xy
300 0.20205766
400 0.27525084
500 0.34751857
600 0.41929803
700 0.49078747
800 0.56252389
900 0.63335009
1000 0.70440089
&


==> Figure_eps/final_DOS <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Sun Jul  2 15:01:08 2023"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, 0, 40, 0.5
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.412990, 0.946078, 0.971814
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Energy (meV)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.250000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 5
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Phonon DOS (states/meV/f.u.)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.250000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.1
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.188235293746, 0.956862745039
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden true
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 0.400000
@    s0 symbol color 15
@    s0 symbol pattern 1
@    s0 symbol fill color 15
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 2
@    s0 line linewidth 1.0
@    s0 line color 15
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 15
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "/home/prakash/Desktop/stewart"
@    s0 legend  "Stewart \f{Times-Italic}et al."
@    s1 hidden true
@    s1 type xy
@    s1 symbol 3
@    s1 symbol size 0.400000
@    s1 symbol color 10
@    s1 symbol pattern 1
@    s1 symbol fill color 10
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 2
@    s1 line linewidth 1.0
@    s1 line color 10
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 10
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "/home/prakash/Desktop/Tuberfeld"
@    s1 legend  "Tuberfeld \f{Times-Italic}et al."
@    s2 hidden false
@    s2 type xy
@    s2 symbol 1
@    s2 symbol size 0.400000
@    s2 symbol color 2
@    s2 symbol pattern 1
@    s2 symbol fill color 2
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 2
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 2
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "/home/prakash/Desktop/Work/Paper_1/Vanadium/phonon_CALCULATION/DMFT/Compare/total_dos_DFT.dat"
@    s2 legend  "DFT"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 4
@    s3 symbol size 0.400000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 1
@    s3 line linewidth 1.0
@    s3 line color 4
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "/home/prakash/Desktop/Work/Paper_1/Vanadium/phonon_CALCULATION/DMFT/Compare/total_dos_DMFT.dat"
@    s3 legend  "DFT+DMFT"
@    s4 hidden true
@    s4 type xy
@    s4 symbol 1
@    s4 symbol size 0.400000
@    s4 symbol color 4
@    s4 symbol pattern 1
@    s4 symbol fill color 4
@    s4 symbol fill pattern 1
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 2
@    s4 line linewidth 1.0
@    s4 line color 4
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 4
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "/home/prakash/Desktop/EISENHAUER"
@    s4 legend  "Experimental data [45]"
@    s5 hidden false
@    s5 type xy
@    s5 symbol 1
@    s5 symbol size 0.500000
@    s5 symbol color 1
@    s5 symbol pattern 1
@    s5 symbol fill color 1
@    s5 symbol fill pattern 1
@    s5 symbol linewidth 1.0
@    s5 symbol linestyle 1
@    s5 symbol char 65
@    s5 symbol char font 0
@    s5 symbol skip 0
@    s5 line type 1
@    s5 line linestyle 4
@    s5 line linewidth 1.0
@    s5 line color 1
@    s5 line pattern 1
@    s5 baseline type 0
@    s5 baseline off
@    s5 dropline off
@    s5 fill type 0
@    s5 fill rule 0
@    s5 fill color 1
@    s5 fill pattern 1
@    s5 avalue off
@    s5 avalue type 2
@    s5 avalue char size 1.000000
@    s5 avalue font 0
@    s5 avalue color 1
@    s5 avalue rot 0
@    s5 avalue format general
@    s5 avalue prec 3
@    s5 avalue prepend ""
@    s5 avalue append ""
@    s5 avalue offset 0.000000 , 0.000000
@    s5 errorbar on
@    s5 errorbar place both
@    s5 errorbar color 1
@    s5 errorbar pattern 1
@    s5 errorbar size 1.000000
@    s5 errorbar linewidth 1.0
@    s5 errorbar linestyle 1
@    s5 errorbar riser linewidth 1.0
@    s5 errorbar riser linestyle 1
@    s5 errorbar riser clip off
@    s5 errorbar riser clip length 0.100000
@    s5 comment "/home/prakash/Desktop/data_dos"
@    s5 legend  "Exp. [51]"
@target G0.S0
@type xy
5.5769695 0.38299769
7.9097428 0.38753964
9.6515079 0.38207043
11.53492 0.37216989
12.977761 0.35781199
14.42158 0.34456355
15.309558 0.36124448
15.907404 0.37902185
16.359697 0.39679272
16.371419 0.41010623
17.119704 0.43343741
17.13338 0.44896984
17.588603 0.47006909
18.183519 0.48451809
18.775504 0.49563871
19.364559 0.50343095
20.665754 0.49350438
21.090694 0.48021039
21.076041 0.4635685
21.342727 0.43584504
21.32612 0.41698423
22.040215 0.40148434
22.167208 0.38041112
22.72598 0.35381013
23.584651 0.33720728
24.297769 0.32059793
25.447549 0.3040081
26.448844 0.28408338
27.023245 0.27523373
27.884847 0.26195927
28.161302 0.24533039
29.016067 0.22428971
30.300655 0.19550233
30.718757 0.17444213
31.135882 0.15227247
31.549099 0.12566497
32.262216 0.10905561
32.976311 0.093555719
33.250812 0.074707926
33.818376 0.058092066
34.829439 0.049261942
&
@target G0.S1
@type xy
3.4022184 0.41954858
4.5795104 0.43054092
5.7477264 0.43380235
6.9107561 0.43264611
8.2154368 0.42817015
9.5071518 0.41265003
10.220593 0.40046906
11.075686 0.38496837
11.631918 0.36285414
12.480527 0.34183137
13.1823 0.31971066
15.365411 0.31961349
16.254215 0.33282762
17.152095 0.35377266
17.904434 0.37472418
18.663255 0.40119778
18.543646 0.42329258
19.00231 0.44204822
19.024352 0.4608233
19.914452 0.47514184
20.484946 0.46517619
21.628527 0.44745371
21.90405 0.43418776
21.75073 0.42756774
21.728688 0.40879267
22.148455 0.39441583
22.130303 0.378954
22.698203 0.36677951
23.546813 0.34575674
23.819743 0.33028196
24.101748 0.32253809
24.808707 0.30483505
25.379201 0.29486939
26.55001 0.30033965
27.557126 0.29035456
27.979486 0.27818655
28.40055 0.26491413
28.964561 0.24942639
29.66763 0.2284101
30.07832 0.20630234
30.785279 0.1885993
30.907481 0.16871333
31.462416 0.14549468
31.87959 0.12890901
32.147333 0.10901656
32.859478 0.095731179
33.556064 0.069192804
34.849076 0.054777097
35.706762 0.041485238
37.592309 0.03587895
39.6221 0.029161768
42.237945 0.025731924
44.853789 0.022302081
46.598982 0.021119934
49.508501 0.019885968
&
@target G0.S2
@type xy
-4.1361998 0
-3.9351541 0
-3.7341085 0
-3.5330629 0
-3.3320172 0
-3.1309716 0
-2.929926 0
-2.7288804 0
-2.5278348 0
-2.3267892 4.8355899e-11
-2.1257436 5.8027079e-10
-1.9246979 6.2137331e-09
-1.7236524 5.2998066e-08
-1.5226067 3.5703578e-07
-1.3215611 1.8986702e-06
-1.1205155 7.9722195e-06
-0.9194699 2.6429545e-05
-0.71842428 6.9180754e-05
-0.51737865 0.00014297684
-0.31633305 0.00023330986
-0.11528744 0.0003006109
0.085758173 0.00030593692
0.28680379 0.00024667662
0.48784939 0.00016168622
0.68889501 0.00010387981
0.88994064 0.00012018726
1.0909862 0.00025397691
1.2920318 0.00053420725
1.4930775 0.0009305462
1.6941231 0.0013324106
1.8951687 0.0016182601
2.0962143 0.0017491117
2.2972599 0.0017546845
2.4983055 0.0016533091
2.6993511 0.0014680785
2.9003968 0.0013138225
3.1014423 0.0013805495
3.302488 0.0018277771
3.5035336 0.0027570261
3.7045792 0.004218441
3.9056248 0.0060536337
4.1066704 0.0077333097
4.307716 0.0086350496
4.5087615 0.0086230319
4.7098071 0.0081316013
4.9108527 0.0075632193
5.1118983 0.0068680626
5.3129443 0.0058902004
5.5139899 0.0049245319
5.7150355 0.0046936074
5.916081 0.0057322926
6.1171266 0.0078286074
6.3181722 0.010130002
6.5192178 0.011858871
6.7202634 0.012886391
6.921309 0.013597081
7.1223545 0.014343745
7.3234001 0.015116518
7.5244457 0.01562994
7.7254913 0.015644846
7.9265369 0.015245451
8.1275829 0.014883096
8.3286285 0.015157063
8.529674 0.016397976
8.7307196 0.018319057
8.9317652 0.020150884
9.1328108 0.021219749
9.3338564 0.021320259
9.534902 0.020545595
9.7359475 0.019116855
9.9369931 0.017708411
10.138039 0.017729301
10.339084 0.020660099
10.54013 0.026600111
10.741175 0.033414664
10.942221 0.03776986
11.143267 0.037619843
11.344313 0.033905974
11.545358 0.029672128
11.746404 0.027541852
11.947449 0.02820705
12.148495 0.030893569
12.349541 0.034402635
12.550586 0.037691117
12.751632 0.040235488
12.952677 0.0420536
13.153723 0.043225955
13.354768 0.043848378
13.555814 0.044622314
13.75686 0.046650967
13.957906 0.050155034
14.158951 0.053942568
14.359997 0.056640597
14.561042 0.058289492
14.762088 0.060459932
14.963134 0.064723346
15.164179 0.070904724
15.365225 0.076888218
15.56627 0.080605353
15.767316 0.082410392
15.968361 0.084970488
16.169407 0.090650375
16.370453 0.099607275
16.571498 0.11027499
16.772544 0.12040117
16.97359 0.1273319
17.174635 0.12894037
17.375681 0.12557081
17.576727 0.1203353
17.777772 0.116366
17.978818 0.11412868
18.179863 0.11239053
18.380909 0.1113114
18.581954 0.11297722
18.783 0.11870266
18.984046 0.12708411
19.185091 0.13498433
19.386137 0.13956641
19.587183 0.13953077
19.788228 0.13585754
19.989274 0.13200566
20.19032 0.13214389
20.391365 0.13782402
20.592411 0.14656313
20.793456 0.15436285
20.994502 0.15928541
21.195547 0.16207656
21.396593 0.16432747
21.597639 0.16764691
21.798684 0.17432253
21.99973 0.18660438
22.200775 0.20389119
22.401821 0.22141096
22.602867 0.23325312
22.803913 0.23701655
23.004958 0.23522099
23.206004 0.23303257
23.407049 0.23509106
23.608095 0.24274383
23.80914 0.25292055
24.010186 0.26109753
24.211232 0.26655783
24.412277 0.27323774
24.613323 0.28404935
24.814368 0.29558206
25.015414 0.30037558
25.21646 0.29470186
25.417506 0.28275766
25.618551 0.27254683
25.819597 0.26880348
26.020642 0.27050592
26.221688 0.27369669
26.422733 0.27528262
26.623779 0.27449587
26.824825 0.27166903
27.02587 0.26625699
27.226916 0.2564213
27.427961 0.24056972
27.629007 0.21919838
27.830053 0.19515411
28.031099 0.17205725
28.232144 0.15244798
28.43319 0.13697622
28.634235 0.12461233
28.835281 0.11365727
29.036326 0.10313565
29.237372 0.093330147
29.438418 0.084998346
29.639463 0.078544662
29.840509 0.074004151
30.041554 0.071151296
30.2426 0.069260887
30.443646 0.067152372
30.644691 0.063886291
30.845737 0.059270181
31.046783 0.053416074
31.247828 0.046159705
31.448874 0.037399773
31.649919 0.027768682
31.850965 0.018544445
32.052011 0.01095365
32.253056 0.0056218697
32.454102 0.0024613919
32.655147 0.0009038463
32.856193 0.00027452067
33.057239 6.8237041e-05
33.258284 1.3773791e-05
33.45933 2.244971e-06
33.660376 2.9422147e-07
33.861421 3.089942e-08
&
@target G0.S3
@type xy
-4.1361998 0
-3.922929 0
-3.7096584 0
-3.4963878 0
-3.2831171 0
-3.0698465 0
-2.8565758 0
-2.6433052 0
-2.4300346 0
-2.2167639 1.6924565e-10
-2.0034933 2.5145068e-09
-1.7902226 2.676499e-08
-1.576952 2.1823017e-07
-1.3636814 1.364265e-06
-1.1504107 6.5375484e-06
-0.93714009 2.4013443e-05
-0.72386948 6.7611219e-05
-0.51059884 0.00014591804
-0.29732818 0.00024139309
-0.084057549 0.00030610218
0.12921309 0.00029753199
0.34248373 0.00022168005
0.55575436 0.00012660336
0.76902501 5.5422945e-05
0.98229566 1.8597703e-05
1.1955663 4.7836074e-06
1.4088369 9.4313346e-07
1.6221076 1.4255319e-07
1.8353782 1.6658607e-08
2.0486489 3.8926499e-09
2.2619195 3.0029014e-08
2.4751901 2.8280948e-07
2.6884608 2.0482834e-06
2.9017314 1.1374541e-05
3.1150021 4.8451789e-05
3.3282727 0.0001584883
3.5415433 0.00039920936
3.754814 0.00077971886
3.9680846 0.0012010515
4.1813554 0.0015160735
4.3946257 0.0016865654
4.6078965 0.0018171434
4.8211673 0.0020050524
5.0344376 0.0022403613
5.2477084 0.0024562635
5.4609792 0.0025670007
5.6742495 0.0024603861
5.8875203 0.0020668618
6.1007911 0.0014657466
6.3140614 0.00087276228
6.5273322 0.00051820733
6.740603 0.00058065704
6.9538733 0.001205463
7.1671441 0.0024245955
7.3804149 0.0039376586
7.5936857 0.0051022031
7.806956 0.0053844367
8.0202268 0.0048309127
8.2334976 0.003977661
8.4467679 0.0034176468
8.6600387 0.0035926663
8.8733095 0.0047207744
9.0865798 0.0065170624
9.2998506 0.0080299028
9.5131214 0.0081846526
9.7263917 0.0067554778
9.9396625 0.0046784219
10.152933 0.003296889
10.366204 0.0034086886
10.579474 0.0049311726
10.792745 0.0070794154
11.006016 0.0088274562
11.219286 0.0096214678
11.432557 0.0097969483
11.645827 0.010088737
11.859098 0.010785662
12.072369 0.011540411
12.285639 0.011830367
12.49891 0.011417192
12.712181 0.0104608
12.925451 0.0093793624
13.138722 0.0087288745
13.351993 0.0091052544
13.565264 0.010869135
13.778534 0.013844845
13.991805 0.017292972
14.205075 0.020106049
14.418346 0.021146061
14.631617 0.019977385
14.844887 0.017675153
15.058158 0.016303305
15.271428 0.016835373
15.484699 0.018005552
15.69797 0.017963166
15.91124 0.016670822
16.124511 0.015952558
16.337782 0.017561269
16.551052 0.021758779
16.764323 0.027264125
16.977593 0.032030745
17.190864 0.034475991
17.404135 0.0344344
17.617405 0.033011407
17.830676 0.031619258
18.043947 0.031029272
18.257217 0.0309931
18.470488 0.030769584
18.683759 0.030287536
18.897029 0.030805575
19.1103 0.034003066
19.323571 0.040040249
19.536841 0.046791533
19.750112 0.051477077
19.963383 0.053002797
20.176653 0.052560907
20.389924 0.052272609
20.603194 0.053627829
20.816465 0.057112882
21.029736 0.062578305
21.243006 0.069140926
21.456277 0.074911064
21.669548 0.077949091
21.882818 0.078307558
22.096089 0.07905205
22.309359 0.08477507
22.52263 0.098563985
22.735901 0.11972405
22.949171 0.14378235
23.162442 0.16466645
23.375713 0.17777901
23.588983 0.18250744
23.802254 0.18271576
24.015525 0.18398821
24.228795 0.18877089
24.442066 0.19405457
24.655337 0.19541928
24.868607 0.19388994
25.081878 0.19668061
25.295149 0.20942987
25.508419 0.22920601
25.72169 0.24714161
25.93496 0.2565163
26.148231 0.25664316
26.361502 0.25154359
26.574772 0.24741538
26.788043 0.24938975
27.001314 0.25849238
27.214584 0.27260471
27.427855 0.29093818
27.641125 0.31555435
27.854396 0.34734669
28.067667 0.38258499
28.280937 0.4147625
28.494208 0.43818409
28.707479 0.44939659
28.920749 0.44783083
29.13402 0.43638443
29.347291 0.41941066
29.560561 0.398442
29.773832 0.37118059
29.987103 0.33622988
30.200373 0.29723385
30.413644 0.26056557
30.626915 0.23013052
30.840185 0.20556577
31.053456 0.18446829
31.266726 0.16546715
31.479997 0.14932197
31.693268 0.13719072
31.906538 0.12821381
32.119809 0.11970474
32.333079 0.10965803
32.54635 0.09804994
32.759621 0.085811274
32.972891 0.073731734
33.186162 0.062430227
33.399433 0.05231896
33.612703 0.043249649
33.825974 0.034635382
34.039245 0.02608933
34.252515 0.017883592
34.465786 0.010810523
34.679057 0.0056035184
34.892327 0.0024305866
35.105598 0.00086428211
35.318869 0.000247772
35.532139 5.6533535e-05
&
@target G0.S4
@type xy
0.097317647 -0.0028831904
2.5302588 0.0028831904
4.4766118 0.0086495713
5.7417412 0.023065523
7.5907765 0.03603988
8.9532235 0.053339023
10.218353 0.070638165
11.191529 0.087937308
12.262024 0.09947007
13.721788 0.11388602
14.792282 0.13406835
16.057412 0.15857547
16.933271 0.18452419
17.711812 0.21768088
18.003765 0.2407464
18.587671 0.26669511
18.976941 0.2998518
19.366212 0.33300849
19.950118 0.35463242
20.923294 0.37913954
21.799153 0.38058114
22.383059 0.36472359
22.480376 0.34598285
23.453553 0.33300849
24.329412 0.34165807
25.107953 0.35607402
25.399906 0.38346433
25.789176 0.40941304
26.762353 0.42527059
27.346259 0.44112813
27.832847 0.44977771
28.903341 0.44401133
29.681882 0.43392016
30.265788 0.41229623
30.460424 0.38490592
30.849694 0.35895721
30.849694 0.34165807
31.044329 0.31859254
31.628235 0.28976064
31.920188 0.25804554
32.406776 0.22921364
32.698729 0.20470652
33.185318 0.181641
33.574588 0.16001707
34.353129 0.13406835
34.839718 0.11532762
35.520941 0.095145284
36.299482 0.079287737
36.883388 0.06919657
&
@target G0.S5
@type xy
1.1160276 0.00095441039
2.1797781 0.0014315092
3.2242549 0.0023765565
4.1161815 0.0042565377
5.1028368 0.0066054305
5.9562841 0.0093042815
6.9800517 0.01317485
8.0977963 0.01880163
8.6275529 0.022668024
9.4421108 0.026887909
10.18053 0.031341205
10.994815 0.036029199
11.695644 0.039780011
12.871415 0.043651863
13.666972 0.047871587
14.158386 0.052322797
14.686844 0.058412709
15.329578 0.064035476
15.858173 0.069891334
16.632611 0.077738742
17.161069 0.083828655
17.896071 0.094133315
18.156336 0.10396585
18.491851 0.11508633
18.883478 0.12772865
19.16329 0.13662513
19.574875 0.14762922
20.121923 0.15442146
20.860548 0.15852367
21.75432 0.15724392
22.155721 0.15315134
22.406349 0.14695098
22.71309 0.14227246
23.152628 0.13794614
23.646844 0.13759923
24.101419 0.14006066
24.592765 0.14462889
24.741488 0.15024749
25.079873 0.15645282
25.398916 0.16324313
25.718369 0.16933128
26.133372 0.17448401
26.511056 0.17846615
26.946084 0.18186363
27.418771 0.18584657
27.96787 0.18912799
28.899643 0.18784855
29.301522 0.18293678
29.761428 0.17627008
30.011783 0.17053783
30.186956 0.16340061
30.418788 0.15684901
30.595328 0.14737125
30.865708 0.13988375
31.060839 0.13110831
31.313244 0.12186524
31.584991 0.1120372
31.990014 0.10174217
32.374192 0.094606721
32.587503 0.08723577
33.02998 0.077877281
33.490911 0.069455171
33.875021 0.062436746
34.450091 0.053781544
35.024068 0.046998779
35.807665 0.039164534
36.972706 0.028875927
&


==> Figure_eps/wth_new_corrected <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Fri Apr 21 18:58:17 2023"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 20, 0, 300, 300
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.393382, 0.970588, 0.966912
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "\f{Times-Italic}T\f{} (K)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.250000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 20
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.200000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place normal
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\f{Symbol}k \f{}(W m\S-1\NK\S-1\N)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.250000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 50
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.200000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.596323529411, 0.956862745098
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 2
@    s0 symbol size 1.000000
@    s0 symbol color 2
@    s0 symbol pattern 1
@    s0 symbol fill color 2
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 3
@    s0 line linewidth 1.0
@    s0 line color 2
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 2
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "/home/prakash/Desktop/Resistivity/WTH/Digitise_thermal_con"
@    s0 legend  "Experimental data [25]"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 1
@    s1 symbol size 1.000000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "/home/prakash/Desktop/Resistivity/WTH/wth_our_300K.dat"
@    s1 legend  "\f{Symbol}k\s\f{Times-Roman}eph\N"
@target G0.S0
@type xy
56.372653 67.669585
66.067104 52.504529
100.15411 37.907235
130.22622 35.646226
151.36089 34.776429
177.37369 33.925171
202.57926 34.496024
226.96989 34.58872
251.36051 34.681416
&
@target G0.S1
@type xy
20 280.21747
40 82.713996
60 48.623046
80 40.133321
100 37.336053
120 36.292978
140 35.892456
160 35.750437
180 35.717364
200 35.730397
220 35.761833
240 35.799155
260 35.836724
280 35.872105
300 35.904385
&

